Improving the Design of Linear Controllers for Homogeneous Platooning under Disturbances

This paper addresses the problem of longitudinal platooning control of homogeneous vehicles subject to external disturbances, such as wind gusts, road slopes, and parametric uncertainties. Our control objective is to maintain the relative distance of the cars regarding their nearby teammates in a decentralized manner. Therefore, we proposed a novel control law to compute the acceleration commands of each vehicle that includes the integral of the spacing error, which endows the controller with the capability to mitigate external disturbances in steady-state conditions. We adopt a constant distance spacing policy and employ generalized look-ahead and bidirectional network topologies. We provide formal conditions for the controller synthesis that ensure the internal stability of the platoon under the proposed control law in the presence of constant and bounded disturbances affecting multiple vehicles. Experiments considering nonlinear vehicle models in the high-fidelity CARLA simulator environment under different disturbances, parametric uncertainties, and several network topologies demonstrate the effectiveness of our approach.

==> Sections/8_acknowledgments.tex <==


% The authors gratefully acknowledge the support for this research provided by FAPESP (Research Grants 2016/04992-6 and 2006/06005-0), FAPEMIG (Research Grant APQ 0913-19), CAPES, CNPq, UFMG, UFSJ, and ITA.

% The Brazilian agencies CAPES, CNPq, and FAPEMIG under the grant APQ 0913-19 have supported this work
% São Paulo Research Foundation (FAPESP)


==> defs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
% operacoes
\newcommand{\escalar}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\vetor}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\matriz}[1]{\ensuremath{\mathbf{\uppercase{#1}}}}
\newcommand{\conjunto}[1]{\ensuremath{\mathcal{\uppercase{#1}}}}
\newcommand{\distribuicao}[1]{\ensuremath{\mathcal{\uppercase{#1}}}}
\newcommand{\transpose}{\ensuremath{{}^\intercal}}

%%%%%%%%%%%%%%%%%%%%%%%%%
% constants
\newcommand{\nrobots}{\escalar{n}}

\newcommand{\dist}[1]{\vetor{\delta}_{#1}}
\newcommand{\xspacing}[1]{\escalar{d}_{#1}}

\newcommand{\vel}{\escalar{v}}
\newcommand{\ivel}[1]{\vel_{#1}}
